MonoScene: Monocular 3D Semantic Scene Completion

MonoScene proposes a 3D Semantic Scene Completion (SSC) framework, where the dense geometry and semantics of a scene are inferred from a single monocular RGB image. Different from the SSC literature, relying on 2.5 or 3D input, we solve the complex problem of 2D to 3D scene reconstruction while jointly inferring its semantics. Our framework relies on successive 2D and 3D UNets bridged by a novel 2D-3D features projection inspiring from optics and introduces a 3D context relation prior to enforce spatio-semantic consistency. Along with architectural contributions, we introduce novel global scene and local frustums losses. Experiments show we outperform the literature on all metrics and datasets while hallucinating plausible scenery even beyond the camera field of view. Our code and trained models are available at https://github.com/cv-rits/MonoScene.

==> Chapters/abstract_cvpr.tex <==
\begin{abstract}
	MonoScene proposes a 3D Semantic Scene Completion (SSC) framework, where the dense geometry and semantics of a scene are inferred from a single monocular RGB image.
	Different from the SSC literature, relying on 2.5 or 3D input, we solve the complex problem of 2D to 3D scene reconstruction while jointly inferring its semantics.
	Our framework relies on successive 2D and 3D UNets bridged by a novel 2D-3D features projection inspiring from optics and introduces a 3D context relation prior to enforce spatio-semantic consistency. Along with architectural contributions, we introduce novel global scene and local frustums losses.
	Experiments show we outperform the literature on all metrics and datasets while hallucinating plausible scenery even beyond the camera field of view. Our code will be opensource.
\end{abstract}

==> Chapters/exp_cvpr.tex <==
\section{Experiments}
We evaluate MonoScene on popular real-world SSC datasets being, indoor NYUv2~\cite{NYUv2} and outdoor SemanticKitti~\cite{behley2019iccv}. 
Because we first address 3D SSC from a 2D image, we detail our non-trivial adaptation of recent SSC baselines~\cite{3DSketch,Li2020aicnet,roldao2020lmscnet,yan2021JS3CNet} (\cref{sec:exp_baselines}) and then detail our performance (\cref{sec:exp_perf}) and ablations (\cref{sec:exp_ablations}).\\

\condenseparagraph{Datasets.}NYUv2~\cite{NYUv2} has 1449 Kinect captured indoor scenes, encoded as 240x144x240 voxel grids labeled with 13 classes (11 semantics, 1 free, 1 unknown). The input RGBD is 640x480.
Similar to~\cite{3DSketch, Li2020aicnet, Li2019ddr, SATNet} we use 795/654 train/test splits and evaluate on the test set at the scale 1:4.

SemanticKITTI~\cite{behley2019iccv} holds outdoor Lidar scans voxelized as 256x256x32 grid of 0.2m voxels, labeled with 21 classes (19 semantics, 1 free, 1 unknown). 
We use RGB image of cam2 of size 1226x370, left cropped to 1220×370.
We use the official 3834/815 train/val splits and always evaluate at full scale (\ie 1:1). Main results are from the hidden test set (online server), and ablations are from the validation set.\\

\condenseparagraph{Training setup.}Unless otherwise mentioned, we use FLoSP at scales (1,2,4,8), 4 supervised relations for 3D~CRP (\ie $n{=}4$, with $\mathcal{L}_{rel}$), and $\ell{\times}\ell{=}8{\times}8$ frustums for $\mathcal{L}_{\text{fp}}$.
We train 30 epochs with an AdamW~\cite{adamW} optimizer, a batch size of 4 and a weight decay of $1\mathrm{e}{\text{-}4}$. The learning rate is $1\mathrm{e}{\text{-}4}$, divided by 10 at epoch 20/25 for NYUv2/SemanticKITTI. For memory reason, the 3D UNet outputs half-size SemanticKITTI and we add a deconv layer in the completion head. Details are in Appendix \ref{sec:3DUnet_detail}.\\

\condenseparagraph{Metrics.}Following common practices, we report the mean intersection over union~(mIoU) of all semantic classes for the SSC task, along with the intersection over union~(IoU) of occupied voxels, regardless of their semantic class, for the scene completion~(SC) task. Note the strong interaction between IoU and mIoU since good geometry estimation (\ie high IoU) can be achieved at the cost of invalid semantic labels (\ie low mIoU).

As mentioned in~\cite{sscsurvey}, the training and evaluation practices differ for indoor (where IoU and mIoU consider only \textit{observed} and \textit{occluded} voxels)
or outdoor settings (considering \textit{all} voxels) due to the different depth/Lidar sparsity. 
As we consider both settings, we use the harder mIoU on \textit{all} voxels. We subsequently retrained all indoor baselines.
\begin{table*}
	\begin{subtable}{1.0\textwidth}
		\scriptsize
		\setlength{\tabcolsep}{0.0045\linewidth}
%		\captionsetup{font=scriptsize}
		\newcommand{\nyuclassfreq}[1]{{~\tiny(\nyufreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c|c c c c c c c c c c c|c}
			\toprule
			& & SC & \multicolumn{12}{c}{SSC} \\[-0.9em]
			Method
			& Input
			& {IoU}
			& \rotatebox{90}{\parbox{2cm}{\textcolor{ceiling}{$\blacksquare$} ceiling\nyuclassfreq{ceiling}}} 
			& \rotatebox{90}{\textcolor{floor}{$\blacksquare$} floor\nyuclassfreq{floor}}
			& \rotatebox{90}{\textcolor{wall}{$\blacksquare$} wall\nyuclassfreq{wall}} 
			& \rotatebox{90}{\textcolor{window}{$\blacksquare$} window\nyuclassfreq{window}} 
			& \rotatebox{90}{\textcolor{chair}{$\blacksquare$} chair\nyuclassfreq{chair}} 
			& \rotatebox{90}{\textcolor{bed}{$\blacksquare$} bed\nyuclassfreq{bed}} 
			& \rotatebox{90}{\textcolor{sofa}{$\blacksquare$} sofa\nyuclassfreq{sofa}} 
			& \rotatebox{90}{\textcolor{table}{$\blacksquare$} table\nyuclassfreq{table}} 
			& \rotatebox{90}{\textcolor{tvs}{$\blacksquare$} tvs\nyuclassfreq{tvs}} 
			& \rotatebox{90}{\textcolor{furniture}{$\blacksquare$} furniture\nyuclassfreq{furniture}} 
			& \rotatebox{90}{\textcolor{objects}{$\blacksquare$} objects\nyuclassfreq{objects}} 
			& mIoU\\
			\midrule
			LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & $\hat{x}^{\text{occ}}$ & 33.93 & 4.49 & 88.41 & 4.63 & 0.25 & 3.94 & 32.03 & 15.44 & 6.57 & 0.02 & 14.51 & 4.39 & 15.88 
			\\
			AICNet$^\text{rgb}$~\cite{Li2020aicnet} & $x^{\text{rgb}}$, $\hat{x}^{\text{depth}}$ & 30.03 & 7.58 & 82.97 & 9.15 & 0.05 & 6.93 & 35.87 & 22.92 & 11.11 & 0.71 & 15.90 & 6.45 & 18.15 
			\\
			3DSketch$^\text{rgb}$~\cite{3DSketch}& $x^{\text{rgb}}$, $\hat{x}^{\text{TSDF}}$  & \underline{38.64} & \underline{8.53} & \underline{90.45} &	\underline{9.94} & \underline{5.67} & \underline{10.64} & \underline{42.29} & \underline{29.21} & \underline{13.88} & \underline{9.38} & \underline{23.83} & \underline{8.19} & \underline{22.91}
			\\
			MonoScene (ours) & $x^{\text{rgb}}$ & \textbf{42.51} & \textbf{8.89} & \textbf{93.50} & \textbf{12.06} & \textbf{12.57} & \textbf{13.72} & \textbf{48.19} & \textbf{36.11} & \textbf{15.13} & \textbf{15.22} & \textbf{27.96} & \textbf{12.94} & \textbf{26.94}\\
			\bottomrule
		\end{tabular}
		\caption{NYUv2 (test set)}
		\label{tab:perf_nyu}
	\end{subtable}
	
	
	\begin{subtable}{1.0\textwidth}
		\scriptsize
%		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.004\linewidth}
		\newcommand{\classfreq}[1]{{~\tiny(\semkitfreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c|c c c c c c c c c c c c c c c c c c c|c}
			\toprule
			& & SC & \multicolumn{20}{c}{SSC} \\
			Method
			& SSC Input
			& {IoU}
			& \rotatebox{90}{\textcolor{road}{$\blacksquare$} road\classfreq{road}} 
			& \rotatebox{90}{\textcolor{sidewalk}{$\blacksquare$} sidewalk\classfreq{sidewalk}}
			& \rotatebox{90}{\textcolor{parking}{$\blacksquare$} parking\classfreq{parking}} 
			& \rotatebox{90}{\textcolor{other-ground}{$\blacksquare$} other-grnd\classfreq{otherground}} 
			& \rotatebox{90}{\textcolor{building}{$\blacksquare$} building\classfreq{building}} 
			& \rotatebox{90}{\textcolor{car}{$\blacksquare$} car\classfreq{car}} 
			& \rotatebox{90}{\textcolor{truck}{$\blacksquare$} truck\classfreq{truck}} 
			& \rotatebox{90}{\textcolor{bicycle}{$\blacksquare$} bicycle\classfreq{bicycle}} 
			& \rotatebox{90}{\textcolor{motorcycle}{$\blacksquare$} motorcycle\classfreq{motorcycle}} 
			& \rotatebox{90}{\textcolor{other-vehicle}{$\blacksquare$} other-veh.\classfreq{othervehicle}} 
			& \rotatebox{90}{\textcolor{vegetation}{$\blacksquare$} vegetation\classfreq{vegetation}} 
			& \rotatebox{90}{\textcolor{trunk}{$\blacksquare$} trunk\classfreq{trunk}} 
			& \rotatebox{90}{\textcolor{terrain}{$\blacksquare$} terrain\classfreq{terrain}} 
			& \rotatebox{90}{\textcolor{person}{$\blacksquare$} person\classfreq{person}} 
			& \rotatebox{90}{\textcolor{bicyclist}{$\blacksquare$} bicyclist\classfreq{bicyclist}} 
			& \rotatebox{90}{\textcolor{motorcyclist}{$\blacksquare$} motorcycl.\classfreq{motorcyclist}} 
			& \rotatebox{90}{\textcolor{fence}{$\blacksquare$} fence\classfreq{fence}} 
			& \rotatebox{90}{\textcolor{pole}{$\blacksquare$} pole\classfreq{pole}} 
			& \rotatebox{90}{\textcolor{traffic-sign}{$\blacksquare$} traf.-sign\classfreq{trafficsign}} 
			& mIoU\\
			\midrule
			LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & $\hat{x}^{\text{occ}}$ &  31.38 & 46.70 & 19.50 & 13.50 & \underline{3.10} & 10.30 & 14.30 & 0.30 & 0.00 & 0.00 & 0.00 & 10.80 & 0.00 & 10.40 & 0.00 & 0.00 & 0.00 & 5.40 & 0.00 & 0.00 & 7.07  \\
			3DSketch$^\text{rgb}$~\cite{3DSketch} & $x^{\text{rgb}}$,$\hat{x}^{\text{TSDF}}$ & 26.85 & 37.70 & 19.80 & 0.00 & 0.00 & 12.10 & 17.10 & 0.00 & 0.00 & 0.00 & 0.00 & 12.10 & 0.00 & \underline{16.10} & 0.00 & 0.00 & 0.00 & 3.40 & 0.00 & 0.00 & 6.23  \\
			AICNet$^\text{rgb}$~\cite{Li2020aicnet} & $x^{\text{rgb}}$,$\hat{x}^{\text{depth}}$ & 23.93	& 15.30	& 0.00	& 0.00	& 0.70	& 0.00	& 0.00	& 0.00	& 0.00	& \textbf{39.30}	& 19.80	& \textbf{18.30}	& 1.60	& {9.60}	& \textbf{5.00}	& \textbf{9.60}	& \textbf{1.90}	& \textbf{13.50}	& 0.10	& 0.00	& 7.09 \\
			*JS3C-Net$^\text{rgb}$~\cite{yan2021JS3CNet} & $\hat{x}^{\text{pts}}$& \underline{34.00} & \underline{47.30} & \underline{21.70} & \underline{19.90} & 2.80 & \underline{12.70} & \textbf{20.10} & \underline{0.80} & 0.00 & 0.00 & \underline{4.10} & {14.20} & \textbf{3.10} & 12.40 & 0.00 & {0.20} & {0.20} & {8.70} & \underline{1.90} & \underline{0.30} & \underline{8.97}  \\
			MonoScene (ours) & $x^{\text{rgb}}$ & \textbf{34.16} & \textbf{54.70} & \textbf{27.10} & \textbf{24.80} & \textbf{5.70} & \textbf{14.40} & \underline{18.80} & \textbf{3.30} & \textbf{0.50} & \underline{0.70} & \textbf{4.40} & \underline{14.90} & \underline{2.40} & \textbf{19.50} & \underline{1.00} & \underline{1.40} & \underline{0.40} & \underline{11.10} & \textbf{3.30} & \textbf{2.10} & \textbf{11.08} \\
			\bottomrule
		\end{tabular}\\
		{* Uses pretrained semantic segmentation network.}
		\caption{Semantic KITTI (hidden test set)}
		\label{tab:perf_semkitti}
	\end{subtable}
	\caption{\textbf{Performance on \subref{tab:perf_nyu} NYUv2~\cite{NYUv2} and \subref{tab:perf_semkitti} SemanticKITTI~\cite{behley2019iccv}.} We report the performance on semantic scene completion (SSC - mIoU) and scene completion (SC - IoU) for RGB-inferred baselines and our method. Despite the various indoor and outdoor setups, we significantly outperform other RGB-inferred baselines, in both mIoU and IoU.}
	\label{tab:perf}
\end{table*}
\subsection{Baselines}\label{sec:exp_baselines}
We consider 4 main SSC baselines among the best opensource ones available -- selecting two indoor-designed methods, 3DSketch~\cite{3DSketch} and AICNet~\cite{Li2020aicnet}, and two outdoor-designed, LMSCNet~\cite{roldao2020lmscnet} and JS3CNet~\cite{yan2021JS3CNet}. Additionally, we also locally compare against S3CNet~\cite{Cheng2020S3CNetAS}, Local-DIFs~\cite{localDif}, CoReNet~\cite{Popov2020CoReNetC3}.

We evaluate baselines in their 3D-input version and main baselines also in an RGB-inferred version.\\

\condenseparagraph{RGB-inferred baselines.}
Unlike us, all baselines need a 3D input \eg occupancy grid, point cloud or depth map, providing them an unfair geometric advantage. 
For fair comparison, we adapt the main baselines to infer their 3D inputs directly from the 2D image ($x^\text{rgb}$) -- relying on the best found methods --, coined as `RGB-inferred' and denoted with a superscript, \eg AICNet$^\text{rgb}$.
Importantly, note that baselines are unchanged. The predicted 3D inputs are denoted with a hat, eg. $\hat{x}^{\text{depth}}$.

We use the pretrained AdaBin~\cite{bhat_adabins_2021} to infer a depth map ($\hat{x}^{\text{depth}}$) serving as input for AICNet$^\text{rgb}$.
Using intrinsic calibration, we further converted depth to TSDF ($\hat{x}^{\text{TSDF}}$) with~\cite{zeng20163dmatch} for 3DSketch$^\text{rgb}$ input, and unproject depth to get a point cloud ($\hat{x}^{\text{pts}}$) directly used as input for JS3CNet$^\text{rgb}$ or discretized as occupancy grid ($\hat{x}^{\text{occ}}$) input for LMSCNet$^\text{rgb}$.
For training \textit{only}, JS3CNet$^\text{rgb}$ also requires a semantic point cloud ($\hat{x}^{\text{sem pts}}$), obtained by augmenting $\hat{x}^{\text{pts}}$ with 2D semantic labels from a pretrained network~\cite{zhu2019labelrelaxation}.
\subsection{Performance}\label{sec:exp_perf}
\subsubsection{Evaluation}
\cref{tab:perf} reports performance of MonoScene and RGB-inferred baselines for NYUv2 (test set) and SemanticKITTI official benchmark (hidden test set).
The low numbers for all methods advocate for task complexity.

On both datasets we outperform all methods by a significant mIoU margin of +4.03 on NYUv2 (\cref{tab:perf_nyu}) and +2.11 on SemanticKITTI (\cref{tab:perf_semkitti}). 
Importantly, the IoU is improved or on par (+3.87 and +0.16) which demonstrates our network captures the scene geometry while avoiding naively increasing the mIoU by lowering the IoU.
On individual classes, MonoScene performs either best or second, excelling on large structural classes for both datasets (\eg floor, wall ; road, building). 
On SemanticKITTI we get outperformed mostly on small moving objects classes (car, motorcycle, person, etc.) which we ascribe to the aggregation of moving objects in the ground truth, highlighted in~\cite{sscsurvey,localDif}. This forces to predict the individual object's motion which we argue is eased when using a 3D input.\\
\begin{figure*}
	\begin{subfigure}{\linewidth}		
		\centering
		\footnotesize
		\renewcommand{\arraystretch}{0.0}
		\setlength{\tabcolsep}{0.003\textwidth}
		\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
		\begin{tabular}{P{0.11\textwidth} P{0.13\textwidth} P{0.13\textwidth} P{0.13\textwidth} P{0.13\textwidth} P{0.13\textwidth}}
			Input & LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & AICNet$^\text{rgb}$~\cite{Li2020aicnet} & 3DSketch$^\text{rgb}$~\cite{3DSketch} & MonoScene \scriptsize{(ours)} & Ground Truth
			\\
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_color.jpg} & 
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_lmscnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_aicnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_sketch.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_our.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU1250_0000_2_gt.png}
			\\		
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_color.jpg} & 
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_lmscnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_aicnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_sketch.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_our.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0994_0000_2_gt.png}
			\\	 	 
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_color.jpg} & 
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_lmscnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_aicnet.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_sketch.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_our.png} &
			\includegraphics[width=\linewidth]{imgs/nyu_qualitative/NYU0970_0000_0_gt.png}
			\\
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{ceiling}{$\blacksquare$}ceiling~
				\textcolor{floor}{$\blacksquare$}floor~
				\textcolor{wall}{$\blacksquare$}wall~
				\textcolor{window}{$\blacksquare$}window~
				\textcolor{chair}{$\blacksquare$}chair~
				\textcolor{sofa}{$\blacksquare$}sofa~
				\textcolor{table}{$\blacksquare$}table~
				\textcolor{tvs}{$\blacksquare$}tvs~
				\textcolor{furniture}{$\blacksquare$}furniture~
				\textcolor{objects}{$\blacksquare$}objects
			}
		\end{tabular}
		\caption{\textbf{NYUv2\cite{NYUv2} (test set).}\\[0.5em]}
		\label{fig:qualitative_NYU}
	\end{subfigure}
	\begin{subfigure}{\linewidth}	
		\centering
		\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
		\setlength{\tabcolsep}{0.001\textwidth}
		\renewcommand{\arraystretch}{0.8}
		\footnotesize
		\begin{tabular}{P{0.157\textwidth} P{0.157\textwidth} P{0.157\textwidth} P{0.157\textwidth} P{0.157\textwidth} P{0.157\textwidth}}		
			Input & AICNet$^\text{rgb}$~\cite{Li2020aicnet} & LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet}  & JS3CNet$^\text{rgb}$~\cite{yan2021JS3CNet}  & \OurMethod\ \scriptsize{(ours)} & Ground Truth
			\\
			\includegraphics[width=.9\linewidth]{imgs/kitti_qualitative/001385.png} &  
			\includegraphics[width=.9\linewidth]{imgs/kitti_qualitative/001385_0_aicnet.png} & 
			\includegraphics[width=.9\linewidth]{imgs/kitti_qualitative/001385_0_lmscnet.png} & 
			\includegraphics[width=.9\linewidth]{imgs/kitti_qualitative/001385_0_js3cnet.png} & 
			\includegraphics[width=.9\linewidth]{imgs/kitti_qualitative/001385_0_our.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001385_0_gt.png} 
			\\
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295_0_aicnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295_0_lmscnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295_0_js3cnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295_0_our.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/000295_0_gt.png} 
			\\
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/002505.png} & 
			\includegraphics[width=0.8\linewidth]{imgs/kitti_qualitative/002505_0_aicnet.png} & 
			\includegraphics[width=0.7\linewidth]{imgs/kitti_qualitative/002505_0_lmscnet.png} & 
			\includegraphics[width=0.7\linewidth]{imgs/kitti_qualitative/002505_0_js3cnet.png} & 
			\includegraphics[width=0.8\linewidth]{imgs/kitti_qualitative/002505_0_our.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/002505_0_gt.png} 
			\\
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005_0_aicnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005_0_lmscnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005_0_js3cnet.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005_0_our.png} & 
			\includegraphics[width=\linewidth]{imgs/kitti_qualitative/001005_0_gt.png} 
			\\		
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{bicycle}{$\blacksquare$}bicycle~
				\textcolor{car}{$\blacksquare$}car~
				\textcolor{motorcycle}{$\blacksquare$}motorcycle~
				\textcolor{truck}{$\blacksquare$}truck~
				\textcolor{other-vehicle}{$\blacksquare$}other vehicle~
				\textcolor{person}{$\blacksquare$}person~
				\textcolor{bicyclist}{$\blacksquare$}bicyclist~
				\textcolor{motorcyclist}{$\blacksquare$}motorcyclist~
				\textcolor{road}{$\blacksquare$}road~
				\textcolor{parking}{$\blacksquare$}parking~}\\
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{sidewalk}{$\blacksquare$}sidewalk~
				\textcolor{other-ground}{$\blacksquare$}other ground~
				\textcolor{building}{$\blacksquare$}building~
				\textcolor{fence}{$\blacksquare$}fence~
				\textcolor{vegetation}{$\blacksquare$}vegetation~
				\textcolor{trunk}{$\blacksquare$}trunk~
				\textcolor{terrain}{$\blacksquare$}terrain~
				\textcolor{pole}{$\blacksquare$}pole~
				\textcolor{traffic-sign}{$\blacksquare$}traffic sign			
			}
		\end{tabular}		
		\caption{\textbf{SemanticKITTI~\cite{behley2019iccv} (val set).}}
		\label{fig:qualitative_kitti}
	\end{subfigure}
	\caption{\textbf{Outputs on~\subref{fig:qualitative_NYU} NYUv2~\cite{NYUv2} and~\subref{fig:qualitative_kitti} SemanticKITTI~\cite{behley2019iccv}.} 
		In both, the input is shown left and the camera viewing frustum is shown in the ground truth (rightmost) with darker colors being parts of scenes \emph{unseen} by the image in~\subref{fig:qualitative_kitti}.
		MonoScene better captures the scene layout on both datasets. On indoor scene~\subref{fig:qualitative_NYU}, it reconstructs thin objects like table legs (row 1), painting and tv (row 2), while in outdoor~\subref{fig:qualitative_kitti}, it better estimates occluded geometry \eg car (row 1--3) and better hallucinates the scenery beyond the field of view (row 1--4).}
	\label{fig:qualitative}
\end{figure*} 

\condenseparagraph{Qualitative.}We compare our SSC outputs in Fig.~\ref{fig:qualitative} showing the input image (leftmost column) and its corresponding camera frustum in ground truth (rightmost).
Notice the noisy labels in NYUv2 having missing objects (\eg windows, rows~2; ceiling, row~3), and in SemanticKITTI having sparse geometry (\eg holes in buildings, rows~1--3).

On indoor scenes (NYUv2, \cref{fig:qualitative_NYU}), all methods correctly capture global scene layouts though only MonoScene recovers thin elements as table legs and cushions (row~1), or the painting frame and properly sized TV (row~2). 

On complex cluttered outdoor scenes (SemanticKITTI, \cref{fig:qualitative_kitti}), compared to baselines, MonoScene evidently captures better the scene layout, \eg cross-roads (rows~1,3).
It also infers finer occluded geometry which is apparent with cars in rows 1--3 having better shapes.
Interestingly, despite a narrow camera field of view (FOV) with respect to the scene, MonoScene properly hallucinates scenery not imaged, \ie \textit{outside} of the camera FOV (darker voxels). This is striking in rows 3,4 where the bottom part of the scene is reasonably guessed, though not in the viewing frustum.
\begin{table}
	\centering
	\begin{subtable}{0.48\linewidth}
		\scriptsize
		\setlength{\tabcolsep}{0.009\linewidth}
%		\captionsetup{font=scriptsize}
		\newcommand{\nyuclassfreq}[1]{{~\tiny(\nyufreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c c}
			\toprule
			Method
			& Input
			& {IoU}	
			& mIoU\\
			\midrule
			\textbf{2.5/3D} &&&\\[-0.1em]
			LMSCNet~\cite{roldao2020lmscnet} & $x^{\text{occ}}$ & \underline{44.1} & 20.4
			\\
			AICNet~\cite{Li2020aicnet} & $x^{\text{rgb}}$, $x^{\text{depth}}$ & 43.8 & 23.8
			\\
			3DSketch~\cite{3DSketch}& $x^{\text{rgb}}$, $x^{\text{TSDF}}$  & \textbf{49.5} & \textbf{29.2}
			\\
			\midrule
			\textbf{2D} &&&\\[-0.1em]
			MonoScene & $x^{\text{rgb}}$ & {42.5} & \underline{26.9}\\
			\bottomrule
		\end{tabular}
		\caption{NYUv2 (test set)}
		\label{tab:perf3d_nyu}
	\end{subtable}\hfill%
	\begin{subtable}{0.48\linewidth}
		\scriptsize
%		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.009\linewidth}
		\newcommand{\classfreq}[1]{{~\tiny(\semkitfreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c c}
			\toprule
			Method & Input & {IoU} & mIoU\\
			\midrule
			\textbf{3D} & & &\\[-0.1em]
			LMSCNet~\cite{roldao2020lmscnet} & $x^{\text{occ}}$ & \underline{56.7} & 17.6	
			\\
			Local-DIFs~\cite{localDif} & $x^{\text{occ}}$ & \textbf{57.7} & 22.7
			\\
			JS3C-Net~\cite{yan2021JS3CNet} & $x^{\text{pts}}$ & 56.6 & \underline{23.8}
			\\
			S3CNet~\cite{Cheng2020S3CNetAS} & $x^{\text{occ}}$ & 45.6 & \textbf{29.5}
			\\
			\midrule
			\textbf{2D} &&&\\[-0.1em]
			MonoScene & $x^{\text{rgb}}$ & {34.2} & {11.1} \\
			\bottomrule
		\end{tabular}\\
		\caption{Semantic KITTI (hidden test set)}
		\label{tab:perf3d_semkitti}
	\end{subtable}
	\caption{\textbf{2.5/3D input baselines}. Despite a single RGB, MonoScene still outperforms the mIoU of \textit{some} indoor baselines.} 
	\label{tab:perf3d}
\end{table}
\subsubsection{Comparison against 2.5/3D-input baselines}
For completeness, we also compare with some original baselines (\ie using real 3D input) in~\cref{tab:perf3d}.
Despite the unfair setup since we use only RGB, in NYUv2 (\cref{tab:perf3d_nyu}) we still beat the recent LMSCNet and AICNet in mIoU by a comfortable margin (+6.48 and +3.17), but with a lower IoU (-1.6 and -1.26). Of note AICNet also uses RGB in addition to depth, showing our method excels at recovering geometry from image only. 
3DSketch, using RGB + TSDF, outperforms us on both mIoU and IoU showing the benefit of TSDF for SSC as mentioned in~\cite{sscsurvey}.
In SemanticKITTI (\cref{tab:perf3d_semkitti}), the baselines clearly surpass us in all metrics which relates both to the lidar-originated 3D input having a much wider horizontal FOV than the camera ($180^{\circ}$ vs $82^{\circ}$), and to the far more complex and cluttered outdoor scenes -- thus harder to reconstruct from a single image viewpoint.
\begin{table}
	\centering
	\setlength{\tabcolsep}{0.015\linewidth}
	\centering
	\footnotesize
	\begin{tabular}{l|cc|cc}
		\toprule
		& \multicolumn{2}{c}{NYUv2} & \multicolumn{2}{c}{SemanticKITTI} \\
		& IoU $\uparrow$ & mIoU $\uparrow$ & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
		Ours &  \underline{42.51} \tiny$\pm$0.15 & \textbf{26.94} \tiny$\pm$0.10 & \textbf{37.12} \tiny$\pm$0.15 & \textbf{11.50} \tiny$\pm$0.14				
		\\
		Ours w/o FLoSP & 28.39 \tiny$\pm$0.53 & 14.11 \tiny$\pm$0.21 & 27.55 \tiny$\pm$0.87 & 4.78\tiny$\pm$0.10
		\\
		Ours w/o 3D CRP & 41.39	\tiny$\pm$0.08  & 26.27 \tiny$\pm$0.15 & 36.20  \tiny$\pm$0.19 & 10.96 \tiny$\pm$0.21
		\\
		Ours w/o $\mathcal{L}^{\text{sem}}_{\text{scal}}$ & \textbf{42.82} \tiny$\pm$0.22 & 25.33 \tiny$\pm$0.26 & \underline{36.78} \tiny$\pm$0.34 & 9.89 \tiny$\pm$0.11				
		\\
		Ours w/o $\mathcal{L}^{\text{geo}}_{\text{scal}}$  & 40.96 \tiny$\pm$0.28 & 26.34 \tiny$\pm$0.23 & 34.92 \tiny$\pm$0.34 & \underline{11.35} \tiny$\pm$0.22				
		\\
		Ours w/o $\mathcal{L}_{\text{fp}}$  & 41.90 \tiny$\pm$0.26 & \underline{26.37} \tiny$\pm$0.16 & 36.74 \tiny$\pm$0.33 & 11.11 \tiny$\pm$0.24  \\
		\bottomrule
	\end{tabular}
	\caption{\textbf{Architecture ablation.} Our components boost performance on NYUv2~\cite{NYUv2} (test set) and SemanticKitti~\cite{behley2019iccv} (val. set).}
	\label{tab:general_ablation}
\end{table}

\subsection{Ablation studies}
\label{sec:exp_ablations}
We ablate our MonoScene framework on both NYUv2 (test set) and SemanticKITTI (validation set), and report the average of 3 runs to account for training variability.

\condenseparagraph{Architectural components.}In \cref{tab:general_ablation} we ablate each component, showing that globally all components contribute to the best performance on both datasets. 
For `w/o FLoSP', we instead interpolate and convolve the 2D decoder features to the required 3D UNet input size. Specifically, FLoSP~(\cref{sec:unprojection}) is shown to be the most crucial as it improves remarkably both semantics ($[+12.83$,$+6.72]$ mIoU) and geometry ($[+14.11$,$+9.56]$ IoU). 3D CRP~(\cref{sec:context_prior}) contributes equally to IoU (in $[+0.77$,$+1.12]$) and mIoU (in $[+0.54, +1.33]$). Our two SCAL losses (\cref{sec:global_loss}) contribute differently as expected, since $\mathcal{L}^{\text{sem}}_{\text{scal}}$ helps semantics ($+1.61$ mIoU in both), while $\mathcal{L}^{\text{geo}}_{\text{scal}}$ boosts geometry ($[+1.55, +2.20]$ IoU). In NYUv2 only, $\mathcal{L}^{\text{sem}}_{\text{scal}}$ harms IoU (-0.31) but improves the same metric on SemanticKITTI (+0.34). 
Finally, the frustums proportion loss~(\cref{sec:frustum_loss}) boosts both metrics on both datasets by at least $+0.38$ and up to $+0.61$.
\begin{table}
	\footnotesize
	\begin{subtable}[b]{0.46\linewidth}
		\centering
%		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.01\linewidth}
		\begin{tabular}[b]{l|cc}
			\toprule
			\makecell{2D scales\\[-0.4em]\scriptsize{~($S$)}} & IoU $\uparrow$ & mIoU $\uparrow$ \\
			\midrule
			$1, 2, 4, 8$ & \textbf{42.51} \tiny$\pm$0.15 & \textbf{26.94} \tiny$\pm$0.10 \\
			$1, 2, 4$ & \underline{42.08} \tiny$\pm$0.69 & \underline{26.28} \tiny$\pm$0.24\\
			$1, 2$ & 41.56 \tiny$\pm$0.18 &	25.66 \tiny$\pm$0.21 \\
			$1$ & 41.57 \tiny$\pm$0.11 & 25.61 \tiny$\pm$0.43 \\
			\midrule
			w/o FLoSP & 28.39 \tiny$\pm$0.53 & 14.11 \tiny$\pm$0.21 \\
			\bottomrule
		\end{tabular}
		\caption{Scales in FLoSP}
		\label{tab:ablate_unprojection}
	\end{subtable}\hfill%
	\begin{subtable}[b]{0.49\linewidth}
		\centering
%		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.01\linewidth}
		\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
		\begin{tabular}[b]{P{0.1\linewidth}|c|cc}
			\toprule
			$n$ & $\mathcal{L}_{rel}$ & IoU $\uparrow$ & mIoU $\uparrow$ \\
			\midrule
			\multirow{2}{*}{4} & \cmark & \textbf{42.51} \tiny$\pm$0.15 & \textbf{26.94} \tiny$\pm$0.10 \\
			& \xmark & \underline{42.24} \tiny$\pm$0.15 &	26.55 \tiny$\pm$0.29 \\
			\midrule
			\multirow{2}{*}{2}  & \cmark & 42.09 \tiny$\pm$0.15 & \underline{26.63} \tiny$\pm$0.05 \\
			& \xmark & 42.15 \tiny$\pm$0.26 & 26.47 \tiny$\pm$0.16 \\
			\midrule
			\multicolumn{2}{c|}{w/o 3D CRP} & 41.39 \tiny$\pm$0.08 & 26.27 \tiny$\pm$0.15 \\
			\bottomrule
		\end{tabular}
		\caption{Relations and supervision in 3D CRP}
		\label{tab:ablation_CP3D}
	\end{subtable}
	\caption{\textbf{Study of FLoSP and 3D CRP.} \subref{tab:ablate_unprojection} Projecting from different 2D scales ($S$) in FLoSP (\cref{sec:unprojection}) show more scales is better. \subref{tab:ablation_CP3D} In our 3D CRP (\cref{sec:context_prior}) using more relations ($n$) and supervision ($\mathcal{L}_{rel}$) lead to higher metrics. Results are on NYUv2.}
	\label{tab:temps}
\end{table}
\begin{figure}
	\centering
	\begin{subfigure}[m]{0.37\linewidth}
		\centering
		\scriptsize
%		\captionsetup{font=scriptsize}
		\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
		\setlength{\tabcolsep}{0.02\linewidth}
		\begin{tabular}{P{0.05\linewidth}c}
			\rotatebox{90}{CoReNet}&\includegraphics[width=0.63\linewidth]{imgs/corenet_compare_corenet.pdf}\\
			\rotatebox{90}{Ours-light}&\includegraphics[width=0.93\linewidth]{imgs/corenet_compare_ours.pdf}\\
		\end{tabular}
		\caption{Architectures ({\textcolor{blue}{2D}} or {\textcolor{red}{3D}})}
		\label{fig:corenet_comparison_arch}
	\end{subfigure}\hfill%
	\begin{subfigure}[m]{0.55\linewidth}
		\centering
		\centering
		\footnotesize
%		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.01\linewidth}
		\begin{tabular}{l|cc}
			\toprule
			& IoU $\uparrow$ & mIoU $\uparrow$ 
			\\
			\midrule
			CoReNet \scriptsize{(1,2,4)} & 30.60 \tiny$\pm$0.46 & 17.34 \tiny$\pm$0.37
			\\
			Ours-light \scriptsize{(1,2,4)} & \textbf{40.80} \tiny$\pm$0.43 & \textbf{25.90} \tiny$\pm$0.63
			\\
			\midrule
			Ours-light \scriptsize{(1)} & 40.13 \tiny$\pm$0.31 & 25.33 \tiny$\pm$0.58
			\\
			\bottomrule
		\end{tabular}
		\caption{Performance}
		\label{fig:corenet_comparison_perf}
	\end{subfigure}
	\caption{\textbf{Type of 2D-3D features projections.} \subref{fig:corenet_comparison_arch} Comparing our FLoSP and `Ray-traced skip connections' from CoReNet~\cite{Popov2020CoReNetC3} (cf. text) shows in \subref{fig:corenet_comparison_perf} we get significantly better results at comparable (1,2,4) scales or even with only one (1).} 
	\label{fig:corenet_comparison}
\end{figure}

\condenseparagraph{Effect of features projection.}We now study in-depth the effect of FLoSP (\cref{sec:unprojection}) at the core our RGB-based task.
In \cref{tab:ablate_unprojection}, we use our FLoSP projecting only 2D features from given 2D scales by changing $S$ in \cref{eq:project2d3d}. More 2D scales boosts IoU and mIoU consistently and leans to lower variance -- showing (1,2,4,8) projections are indeed best.

We further compare FLoSP to the `Ray-traced skip connections' of CoReNet~\cite{Popov2020CoReNetC3} being close in nature, putting our best effort to push CoReNet performance.
To properly evaluate only the effect of features projection, we remove our other components, producing a light version (`Ours-light') with the same 2D encoder (E), 3D decoder (D), and projection scales (1,2,4), corresponding to all possible scales in the 3D decoder, as in CoReNet, shown in \cref{fig:corenet_comparison_arch}. 
On NYUv2, \cref{fig:corenet_comparison_perf} shows FLoSP is very significantly better (+10.2~IoU, +8.56~mIoU). We conjecture this relates to the fact that CoReNet applies same-scale 2D-3D connections, while FLoSP disentangles 2D-3D scales, letting the network relies on self-learned relevant features, confirmed by the good performance of the (1) scale in \cref{fig:corenet_comparison_perf}.

\condenseparagraph{Effect of relations in 3D CRP.}While 3D Context Relation Prior (\cref{sec:context_prior}) is shown beneficial in \cref{tab:general_ablation}, we evaluate the effect of using different number of relations (\ie~$n$).
\cref{tab:ablation_CP3D} shows the benefit of our 4 relations 
$\mathcal{M}{=}\{\textbf{f}_{\textbf{s}},\textbf{f}_{\textbf{d}},\textbf{o}_{\textbf{s}},\textbf{o}_{\textbf{d}}\}$
instead of only 2 (\ie $\mathcal{M}{=}\{\textbf{s},\textbf{d}\}$),
which matches our expectation due to the overwhelming imbalance of free/occupied voxels ($\approx{}9{:}1$ in NYUv2). 
Our supervision of relation matrices $\hat{A}$ with the relation loss $\mathcal{L}_{rel}$ from \cref{eq:loss_rel} also shows an increase of all metrics. Without supervision, our 3D CRP acts as a self-attention layer that learns the context information implicitly.
\begin{table}
	\centering
	\setlength{\tabcolsep}{0.01\linewidth}
	\centering
	\footnotesize
	\begin{tabular}{l|cc|cc}
		\toprule
		& \multicolumn{2}{c}{NYUv2} & \multicolumn{2}{c}{SemanticKITTI} \\
		$\ell{\times}\ell$ & IoU $\uparrow$ & mIoU $\uparrow$ &  IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule	
		$8 \times 8$ & \underline{42.51} \tiny$\pm$0.15 & \textbf{26.94} \tiny$\pm$0.10 &
		\textbf{37.12} \tiny$\pm$0.15 & \textbf{11.50} \tiny$\pm$0.14
		\\					
		$4 \times 4$ & \textbf{42.52} \tiny$\pm$0.12 & \underline{26.85} \tiny$\pm$0.19 &
		\underline{37.09} \tiny$\pm$0.09 & \underline{11.45} \tiny$\pm$0.15 
		\\
		$2 \times 2$ & 42.41 \tiny$\pm$0.13 & \underline{26.85} \tiny$\pm$0.22 
		& 36.88 \tiny$\pm$0.11 & 11.27 \tiny$\pm$0.25
		\\
		$1 \times 1$ & 42.39 \tiny$\pm$0.18 & 26.52 \tiny$\pm$0.31
		& 36.83 \tiny$\pm$0.42 & 11.33 \tiny$\pm$0.11
		\\									
		\midrule
		w/o $\mathcal{L}_{\text{fp}}$ & 41.90 \tiny$\pm$0.26 & 26.37 \tiny$\pm$0.16 
		& 36.74 \tiny$\pm$0.33 & 11.11 \tiny$\pm$0.24
		\\
		\bottomrule
	\end{tabular}
	\caption{\textbf{Frustums Proportion loss ablation.} Varying the number of local frustums ($\ell{\times}\ell$) in our loss shows more frustums (\ie smaller) lead to finer guidance and better results on both datasets.} 
	\label{tab:frustum_loss_ablation}
\end{table}

\condenseparagraph{Effect of local frustums loss.}\cref{tab:frustum_loss_ablation} shows the effect of varying number of $\ell{\times}\ell$ frustums (\cref{eq:frustum_loss}, \cref{sec:frustum_loss}) on both datasets. 
Higher numbers result in smaller frustums, \ie finer local supervision. As $\ell{\times}\ell$ increases, all metrics increase accordingly, showing the loss benefit, especially when compared to applied image-wise (\ie~$1{\times}1$).


\begin{figure}
	\centering
	\scriptsize
	\setlength{\fboxsep}{0.005pt}
	\newcommand{\tmpframe}[1]{\fbox{#1}}
	\newcommand{\im}[3]{\stackinset{r}{0cm}{b}{0pt}{\tmpframe{\includegraphics[height=#3]{#1}}}{\includegraphics[width=\linewidth]{#2}}} %
	\newcommand{\imcs}[1]{\im{imgs/generalization/cityscapes/#1.png}{imgs/generalization/cityscapes/#1_our.png}{0.5cm}}
	\newcommand{\imns}[1]{\im{imgs/generalization/nuscenes/#1_nclass.jpg}{imgs/generalization/nuscenes/#1_nclass_0_our.png}{0.5cm}}
	\newcommand{\imkt}[1]{\im{imgs/kitti_qualitative/#1.png}{imgs/kitti_qualitative/#1_0_our.png}{0.36cm}}
	\newcommand{\imktnew}[1]{\im{imgs/generalization/kitti360/#1.png}{imgs/generalization/kitti360/#1_0_our.png}{0.35cm}}
	\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
	\setlength{\tabcolsep}{0.01\linewidth}
	\renewcommand{\arraystretch}{0.0}
	\begin{tabular}{P{0.235\linewidth} P{0.235\linewidth} P{0.235\linewidth} P{0.235\linewidth}}		
		Cityscapes~\cite{cityscapes} & 
		Nuscenes~\cite{nuscenes2019} & 
		\textbf{SemanticKITTI~\cite{behley2019iccv}}
		& KITTI-360~\cite{KITTI360}\\
		\imcs{197} & \imns{148} & \imkt{000465} & \imktnew{0000001799}
		\\
		\imcs{393} & \imns{74} & \imkt{002360} & \imktnew{0000006988}\\
		(49$^{\circ}$, 25$^{\circ}$) & (65$^{\circ}$, 39$^{\circ}$) & (H=82$^{\circ}$, V=29$^{\circ}$) & (104$^{\circ}$, 38$^{\circ}$)
		\\
	\end{tabular}
	\caption{\textbf{Camera effects.} Outputs of MonoScene when trained on Sem.KITTI having horizontal FOV of 82$^\circ$, and tested on datasets with decreasing (left) or increasing (right) FOV.}
	\label{fig:fov_generalization}
\end{figure}

==> Chapters/problem_statement.tex <==
% !TEX root = ../main.tex

\section{Problem statement}
\label{sec:probstatement}
%\RCc{This section should focus on your novelty (3D SSC from 2D) rather than redefining the 3D SSC task.}
%\QCc{Agree!}

%may it encoded as voxel occupancy grids~\cite{xx}, point cloud~\cite{xx} or depth data~\cite{xx}
3D Semantic Scene Completion (SSC) aims to infer a dense semantically labeled 3D scene $\hat{y}$. 
While SSC was already addressed with sparse 3D inputs~\cite{sscsurvey}, we instead solve use a single RGB image $x^{\text{RGB}}$. Particularly, we want to learn a function $f$ such that $\hat{y} = f(x^{\text{RGB}})$.
This is significantly harder, since even sparse 3D input provide a strong 
\begin{equation}
	\hat{y} = f(x^{\text{RGB}})\,.
\end{equation} 
%While the literature has addressed from sparse 3D input originating from depth or Lidar scans (optionally with additional RGB), we chose to 

% sometimes along optional RGB data $x^{\text{RGB}}$. 
%Because 3D geometry is a subset of 3D semantics -- since all non-free class resolves as occupied -- $x_{\text{3D}}$ acts as a strong geometric clue for the network.

%Instead, in this work we want to infer the complete 3D geometry and semantic from a single RGB image $x^{\text{RGB}}$. Particularly, we want to learn a function $f(\cdot)$ such that
%
\todo{
We refer to this task as \emph{Semantic Scene Completion from single RGB image (SSC2D)}. \RCc{no big fan of this naming}
}
\QCc{To find a name or perhap we should keep this one}
\RCc{I don't think we should name the task, the task is the same as before just the input changed. Also, it lacks consistency since we refer to SSC everywhere else.}

%%%%%%%%% Proposed approach
